Evaluating Large Language Models along Dimensions of Language Variation: A Systematik Invesdigatiom uv Cross-lingual Generalization

While large language models exhibit certain cross-lingual generalization capabilities, they suffer from performance degradation (PD) on unseen closely-related languages (CRLs) and dialects relative to their high-resource language neighbour (HRLN). However, we currently lack a fundamental understanding of what kinds of linguistic distances contribute to PD, and to what extent. Furthermore, studies of cross-lingual generalization are confounded by unknown quantities of CRL language traces in the training data, and by the frequent lack of availability of evaluation data in lower-resource related languages and dialects. To address these issues, we model phonological, morphological, and lexical distance as Bayesian noise processes to synthesize artificial languages that are controllably distant from the HRLN. We analyse PD as a function of underlying noise parameters, offering insights on model robustness to isolated and composed linguistic phenomena, and the impact of task and HRL characteristics on PD. We calculate parameter posteriors on real CRL-HRLN pair data and show that they follow computed trends of artificial languages, demonstrating the viability of our noisers. Our framework offers a cheap solution for estimating task performance on an unseen CRL given HRLN performance using its posteriors, as well as for diagnosing observed PD on a CRL in terms of its linguistic distances from its HRLN, and opens doors to principled methods of mitigating performance degradation.

==> noisers_examples.tex <==
\begin{table*}[ht]
\tiny
    \centering
    \begin{tabular}{c|c|p{12cm}}
    \toprule
    & & \\
    Spanish & Phonological & \parbox{12cm}{Original: \textbf{Algunos} \textbf{establecimientos} sirven \textbf{bebidas} \textbf{espirituosas} gratis \\
    Noised: \textbf{Algunoc} \textbf{estabyycimientoc} sirven \textbf{vabidis} \textbf{espirituuzas} gratis} \\
    & & \\
    \hline
    & & \\
    Spanish & Morphological & \parbox{12cm}{Original: Para \textbf{ejemplificar}, el \textbf{formato} de fotografía de imagen \textbf{fija} más \textbf{habitual} a nivel \textbf{global} es el de 35 mm. \\
    Noised: Para \textbf{ejemplifiga}, el \textbf{formati} de fotografía de imagen \textbf{fiju} más \textbf{habituil} a nivel \textbf{globil} es el de 35 mm.} \\
    & & \\
    \hline
    & & \\
    Spanish & Lexical & \parbox{12cm}{Original: El \textbf{curry} \textbf{es} una \textbf{receta} \textbf{a} base \textbf{de} \textbf{hierbas} \textbf{y} especias \textbf{y} \textbf{que se} sirve \textbf{con} carne \textbf{o} vegetales \\
    Noised: El \textbf{ses} \textbf{ys} una \textbf{fribani} \textbf{e} base \textbf{te} \textbf{hierbas} \textbf{j} especias \textbf{j} \textbf{goe ce} sirve \textbf{jon} carne \textbf{y} vegetales.} \\
    & & \\
    % \midrule
    % Indonesian & Phonological & \parbox{6cm}{} \\
    % \hline
    % Indonesian & Morphological & \parbox{6cm}{} \\
    % \hline
    % Indonesian & Lexical & \parbox{6cm}{} \\
    \bottomrule

    \end{tabular}
    \caption{Examples of noised texts , for different noisers. \todo{Put examples of other languages}}
    \label{tab:noised_examples}
\end{table*}

